Waiting Buys Exactly Two Moments: Endogenous Identification in Prediction-Driven Allocation

A planner with a fixed budget of preventive help must decide whom to help and when. Waiting reveals risk but removes intervention opportunities as higher-risk individuals leave first. We characterize this tradeoff under repeated noisy signals and risk-dependent attrition: in the canonical model, a length-$\tau$ observation prefix identifies exactly the latent risk moments $m_j=\mathbb E[p^j]$ for $j=0,\ldots,2\tau-1$, buying two new moments per additional period. These identify average next-period attrition among survivors but need not identify allocation welfare or attrition among those prioritized for treatment. Our observationally equivalent constructions establish unavoidable timing regret at any sample size for a fixed observation length, while exact certificates determine whether all compatible populations share a unique optimal date. Matched experiments separate the effects of estimation, bootstrap averaging, and regret weighting. Longer observation often resolves timing ambiguity, but the optimal date may already have passed. In our experiments, bootstrap averaging and early stopping improve decisions, while regret weighting adds no improvement in pooled mean squared regret: better statistical fit need not yield better allocation welfare. The code and artifacts are available at https://github.com/KurbanIntelligenceLab/waiting-buys-two-moments.

==> Makefile <==
#===============================================================================
# Kurban Intelligence Lab -- paper build
#
#   make          build main.pdf (pdflatex -> bibtex -> pdflatex x2)
#   make arxiv    arxiv-submission.tar.gz, ready to upload
#   make blind    main-blind.pdf   (double-blind: no authors, no logo, no acks)
#   make logo     regenerate every logo asset from the vector master
#   make figures  regenerate the example figure
#   make clean    remove build artefacts (keeps the PDFs)
#   make purge    remove everything generated
#===============================================================================
MAIN  := main
LATEX := pdflatex -interaction=nonstopmode -halt-on-error

.PHONY: all arxiv blind logo figures clean purge
all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex kurbanlab.sty affiliations.tex references.bib
	$(LATEX) $(MAIN)
	-bibtex $(MAIN)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)
	@echo "==> $(MAIN).pdf"

# arXiv wants the .bbl, not the .bib, and no build cruft.
arxiv: $(MAIN).pdf
	@rm -rf arxiv && mkdir -p arxiv/figures arxiv/logo
	@cp $(MAIN).tex kurbanlab.sty affiliations.tex references.bib .latexmkrc $(MAIN).bbl arxiv/
	@cp figures/*.pdf arxiv/figures/ 2>/dev/null || true
	@cp logo/kil-lockup.pdf arxiv/logo/ 2>/dev/null || true
	@cd arxiv && tar czf ../arxiv-submission.tar.gz .
	@rm -rf arxiv
	@echo "==> arxiv-submission.tar.gz  (upload this)"
	@echo "    contains: $(MAIN).tex, kurbanlab.sty, affiliations.tex, $(MAIN).bbl, figures/, logo/"
	@echo "    NOT included: *.aux, *.log. references.bib IS included: arXiv ignores it,"
	@echo "    but anyone opening this tarball in Overleaf gets a working BibTeX setup."

blind:
	@sed -E 's/\\usepackage\[([^]]*)\]\{kurbanlab\}/\\usepackage[\1, blind]{kurbanlab}/' \
	     $(MAIN).tex > $(MAIN)-blind.tex
	$(LATEX) $(MAIN)-blind
	-bibtex $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	@echo "==> $(MAIN)-blind.pdf  (check it: your name should appear nowhere)"

logo:
	@cd logo && sh build-logo.sh

figures:
	@cd figures && python3 make-figure.py

clean:
	@rm -f *.aux *.log *.out *.bbl *.blg *.toc *.lof *.lot *.fls *.fdb_latexmk \
	       *.synctex.gz *.nav *.snm *.vrb $(MAIN)-blind.tex
	@echo "==> cleaned"

purge: clean
	@rm -f $(MAIN).pdf $(MAIN)-blind.pdf arxiv-submission.tar.gz
	@rm -rf arxiv

